Context-Aware Cross-Lingual Mapping

Cross-lingual word vectors are typically obtained by fitting an orthogonal matrix that maps the entries of a bilingual dictionary from a source to a target vector space. Word vectors, however, are most commonly used for sentence or document-level representations that are calculated as the weighted average of word embeddings. In this paper, we propose an alternative to word-level mapping that better reflects sentence-level cross-lingual similarity. We incorporate context in the transformation matrix by directly mapping the averaged embeddings of aligned sentences in a parallel corpus. We also implement cross-lingual mapping of deep contextualized word embeddings using parallel sentences with word alignments. In our experiments, both approaches resulted in cross-lingual sentence embeddings that outperformed context-independent word mapping in sentence translation retrieval. Furthermore, the sentence-level transformation could be used for word-level mapping without loss in word translation quality.

==> main_figure.tex <==
\begin{figure} [H]
\hspace{-0.2cm}
\begin{subfigure}{0.238\textwidth}
\centering
%\scriptsize
\small
 \begin{tikzpicture}[font=\sffamily, scale=0.80, transform shape]
\begin{semilogyaxis}[title=es $\rightarrow$ en ,
                ymode=normal,
                ymin=0,
                ymax=100,
                xmin=0,
                ytick={20, 50, 80, 100},
                yticklabels={.2, .5, .8, 1},
                xtick={1, 10,100, 1000},
                xticklabels={1K,10K,100K, 1M}, % 
                xmode=log, 
                log basis x={2},
                axis x line=bottom,
                axis y line=left,
                axis line style=-,
                x=0.3cm, y=0.03cm,
                ylabel = NN accuracy,
                compat=newest,
                y label style={at={(-0.1,0.5)}},
                %xlabel = parallel sentences (K)
                ]
\addplot[blue, dotted, mark=*,mark options={solid, scale=0.7}] table [x=size, y=elmo_avg, col sep=space] {es_en.nn};
\addplot[brown,mark=o,mark options={solid, scale=0.7}] table [x=size, y=elmo_sent, col sep=space] {es_en.nn};
\addplot[red, dotted, mark=x,mark options={solid, scale=1, fill=black}] table [x=size, y=siskip_sif, col sep=space] {es_en.nn};
\addplot[green,mark=none,mark options={solid, scale=1}] table [x=size, y=siskip_sent, col sep=space] {es_en.nn};
\addplot [dashed] table [x=size, y=muse_sif, col sep=space] {es_en.nn};
\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}% 
\hspace{0.1cm}
\begin{subfigure}{0.238\textwidth}
\centering
\small

 \begin{tikzpicture}[font=\sffamily, scale=0.80, transform shape]
\begin{semilogyaxis}[title=de $\rightarrow$ en ,
               % legend pos=outer north east,
                %legend style={draw=none},
                ymode=normal,
                ymin=0,
                ymax=100,
                xmin=0,
                 ytick={20, 50, 80, 100},
                yticklabels={.2, .5, .8, 1},
                xtick={1, 10,100, 1000},
                xticklabels={1K,10K,100K, 1M}, % 
                xmode=log, 
                log basis x={2},
                axis x line=bottom,
                axis y line=left,
                axis line style=-,
                x=0.3cm, y=0.03cm,
                ]
\addplot[blue, dotted, mark=*,mark options={solid, scale=0.7}] table [x=size, y=elmo_avg, col sep=space] {de_en.nn};
\addplot[brown,mark=o,mark options={solid, scale=0.7}] table [x=size, y=elmo_sent, col sep=space] {de_en.nn};
\addplot[red, dotted, mark=x,mark options={solid, scale=1, fill=black}] table [x=size, y=siskip_sif, col sep=space] {de_en.nn};
\addplot[green,mark=none,mark options={solid, scale=1}] table [x=size, y=siskip_sent, col sep=space] {de_en.nn};
\addplot [dashed] table [x=size, y=muse_sif, col sep=space] {de_en.nn};
\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}\\%

\vspace{0.5cm}
\hspace{-0.2cm}
\begin{subfigure}{0.238\textwidth}
\centering
%\scriptsize
\small
 \begin{tikzpicture}[font=\sffamily, scale=0.80, transform shape]
\begin{semilogyaxis}[title=en $\rightarrow$ es ,
               % legend pos=outer north east,
                %legend style={draw=none},
                 title style={at={(0.5,1.0)},anchor=north,yshift=-0.1},
                ymode=normal,
                ymin=0,
                ymax=100,
                xmin=0,
                 ytick={20, 50, 80, 100},
                yticklabels={.2, .5, .8, 1},
                xtick={1, 10,100, 1000},
                xticklabels={1K,10K,100K, 1M}, % 
                xmode=log, 
                log basis x={2},
                axis x line=bottom,
                axis y line=left,
                axis line style=-,
                x=0.3cm, y=0.03cm,
                ylabel = NN accuracy,
                compat=newest,
                y label style={at={(-0.1,0.5)}},
                ]
\addplot[blue, dotted, mark=*,mark options={solid, scale=0.7}] table [x=size, y=elmo_avg, col sep=space] {en_es.nn};
\addplot[brown,mark=o,mark options={solid, scale=0.7}] table [x=size, y=elmo_sent, col sep=space] {en_es.nn};
\addplot[red, dotted, mark=x,mark options={solid, scale=1, fill=black}] table [x=size, y=siskip_sif, col sep=space] {en_es.nn};
\addplot[green,mark=none,mark options={solid, scale=1}] table [x=size, y=siskip_sent, col sep=space] {en_es.nn};
\addplot [dashed] table [x=size, y=muse_sif, col sep=space] {en_es.nn};
\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}% 
\hspace{0.1cm}
\begin{subfigure}{0.238\textwidth}
\centering
\small

 \begin{tikzpicture}[font=\sffamily, scale=0.80, transform shape]
\begin{semilogyaxis}[title=en $\rightarrow$ de ,
                ymode=normal,
                 title style={at={(0.5,1.0)},anchor=north,yshift=-0.1},
                ymin=0,
                ymax=100,
                xmin=0,
                 ytick={20, 50, 80, 100},
                yticklabels={.2, .5, .8, 1},
                xtick={1, 10,100, 1000},
                xticklabels={1K,10K,100K, 1M}, % 
                xmode=log, 
                log basis x={2},
                axis x line=bottom,
                axis y line=left,
                axis line style=-,
                x=0.3cm, y=0.03cm,
                ]
\addplot[blue, dotted, mark=*,mark options={solid, scale=0.7}] table [x=size, y=elmo_avg, col sep=space] {en_de.nn};
\addplot[brown,mark=o,mark options={solid, scale=0.7}] table [x=size, y=elmo_sent, col sep=space] {en_de.nn};
\addplot[red, dotted, mark=x,mark options={solid, scale=1, fill=black}] table [x=size, y=siskip_sif, col sep=space] {en_de.nn};
\addplot[green,mark=none,mark options={solid, scale=1}] table [x=size, y=siskip_sent, col sep=space] {en_de.nn};
\addplot [dashed] table [x=size, y=muse_sif, col sep=space] {en_de.nn};
\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}%

\vspace{0.5cm}
\hspace{-0.2cm}
\begin{subfigure}{0.238\textwidth}
\centering
%\scriptsize
\small
 \begin{tikzpicture}[font=\sffamily, scale=0.80, transform shape]
\begin{semilogyaxis}[title=es $\rightarrow$ de ,
                 title style={at={(0.5,1.0)},anchor=north,yshift=-0.1},
                ymode=normal,
                ymin=0,
                ymax=100,
                xmin=0,
                 ytick={20, 50, 80, 100},
                yticklabels={.2, .5, .8, 1},
                xtick={1, 10,100, 1000},
                xticklabels={1K,10K,100K, 1M}, % 
                xmode=log, 
                log basis x={2},
                axis x line=bottom,
                axis y line=left,
                axis line style=-,
                x=0.3cm, y=0.03cm,
                ylabel = NN accuracy,
                compat=newest,
                y label style={at={(-0.1,0.5)}},
                xlabel = \# parallel sentences
                ]

\addplot[blue, dotted, mark=*,mark options={solid, scale=0.7}] table [x=size, y=elmo_avg, col sep=space] {es_de.nn};
\addplot[brown,mark=o,mark options={solid, scale=0.7}] table [x=size, y=elmo_sent, col sep=space] {es_de.nn};
\addplot[red, dotted, mark=x,mark options={solid, scale=1, fill=black}] table [x=size, y=siskip_sif, col sep=space] {es_de.nn};
\addplot[green,mark=none,mark options={solid, scale=1}] table [x=size, y=siskip_sent, col sep=space] {es_de.nn};
\addplot [dashed] table [x=size, y=muse_sif, col sep=space] {es_de.nn};
\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}% 
\hspace{0.1cm}
\begin{subfigure}{0.238\textwidth}
\centering
\small

 \begin{tikzpicture}[font=\sffamily, scale=0.80, transform shape]
\begin{semilogyaxis}[title=de $\rightarrow$ es ,
                ymode=normal,
                 title style={at={(0.5,1.0)},anchor=north,yshift=-0.1},
                ymin=0,
                ymax=100,
                xmin=0,
                 ytick={20, 50, 80, 100},
                yticklabels={.2, .5, .8, 1},
                xtick={1, 10,100, 1000},
                xticklabels={1K,10K,100K, 1M}, % 
                xmode=log, 
                log basis x={2},
                axis x line=bottom,
                axis y line=left,
                axis line style=-,
                x=0.3cm, y=0.03cm,
                xlabel = \# parallel sentences
                ]
\addplot[blue, dotted, mark=*,mark options={solid, scale=0.7}] table [x=size, y=elmo_avg, col sep=space] {de_es.nn};
\addplot[brown,mark=o,mark options={solid, scale=0.7}] table [x=size, y=elmo_sent, col sep=space] {de_es.nn};
\addplot[red, dotted, mark=x,mark options={solid, scale=1, fill=black}] table [x=size, y=siskip_sif, col sep=space] {de_es.nn};
\addplot[green,mark=none,mark options={solid, scale=1}] table [x=size, y=siskip_sent, col sep=space] {de_es.nn};
\addplot [dashed] table [x=size, y=muse_sif, col sep=space] {de_es.nn};
%\legend{$a$,$b$,$c$,$d$,$e$}
\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}\\ %%%%%%%%%%%%%%%%%%%
\vspace{1.5pt}
\begin{subfigure}{0.238\textwidth}
\centering
\small
 \begin{tikzpicture}[font=\sffamily, scale=0.8, transform shape]
\begin{semilogyaxis}[title=Average ,
                ymode=normal,
                 title style={at={(0.5,1.0)},anchor=north,yshift=-0.1},
                ymin=0,
                ymax=100,
                xmin=0,
                 ytick={20, 50, 80, 100},
                yticklabels={.2, .5, .8, 1},
                xtick={1, 10,100, 1000},
                xticklabels={1K,10K,100K, 1M}, % 
                xmode=log, 
                log basis x={2},
                axis x line=bottom,
                axis y line=left,
                axis line style=-,
                x=0.3cm, y=0.03cm,
                xlabel = \# parallel sentences
                ]
\addplot[blue, dotted, mark=*,mark options={solid, scale=0.7}] table [x=size, y=elmo_avg, col sep=space] {avg.nn};
\addplot[brown,mark=o,mark options={solid, scale=0.7}] table [x=size, y=elmo_sent, col sep=space] {avg.nn};
\addplot[red, dotted, mark=x,mark options={solid, scale=1, fill=black}] table [x=size, y=siskip_sif, col sep=space] {avg.nn};
\addplot[green,mark=none,mark options={solid, scale=1}] table [x=size, y=siskip_sent, col sep=space] {avg.nn};
\addplot [dashed] table [x=size, y=muse_sif, col sep=space] {avg.nn};
%\legend{$a$,$b$,$c$,$d$,$e$}
\end{semilogyaxis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}{0.21\textwidth}
\small
 \begin{tikzpicture}[font=\sffamily, scale=0.750, transform shape]
\begin{axis}[
    hide axis,
    xmin=0,
    xmax=0.5,
    ymin=0,
    ymax=0.4,
    legend style={at={(0.3,0.8)},anchor=north east,draw=white!15!black,legend cell align=left},
    % legend pos=north middle
    ]
\addlegendimage{blue, dotted, mark=*,mark options={solid, scale=0.7}}
\addlegendentry{ELMo \hspace{9pt}\texttt{(word)} 82.23\%};
\addlegendimage{brown,mark=o,mark options={solid, scale=0.7}}
\addlegendentry{ELMo \hspace{9pt}\texttt{(sent)} 84.03\%};
\addlegendimage{red, dotted, mark=x,mark options={solid, scale=1, fill=black}} 
\addlegendentry{FastText \texttt{(word)} 74.00\%};
\addlegendimage{green,mark=none,mark options={solid, scale=1}}
\addlegendentry{FastText \texttt{(sent)} 76.92\%};
\addlegendimage {dashed}
\addlegendentry{FastText \texttt{(dict)} 69.04\%};
%\legend{$a$,$b$,$c$,$d$,$e$}
\end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{minipage}{0.48\textwidth}
\centering
\caption{Nearest neighbor sentence translation accuracy as a function of (log) parallel corpus size. \texttt{(word)} refers  to word-level mapping, \texttt{(sent)} to sentence-level mapping, and \texttt{(dict)} refers to the baseline (using a static dictionary for mapping). The legend shows the average accuracies of each model using 1M parallel sentences.} \label{fig:nn_acc}
\end{minipage}\hfill
\end{figure}


